Modified-CS: Modifying Compressive Sensing for Problems with Partially Known Support

We study the problem of reconstructing a sparse signal from a limited number of its linear projections when a part of its support is known, although the known part may contain some errors. The ``known" part of the support, denoted T, may be available from prior knowledge. Alternatively, in a problem of recursively reconstructing time sequences of sparse spatial signals, one may use the support estimate from the previous time instant as the ``known" part. The idea of our proposed solution (modified-CS) is to solve a convex relaxation of the following problem: find the signal that satisfies the data constraint and is sparsest outside of T. We obtain sufficient conditions for exact reconstruction using modified-CS. These are much weaker than those needed for compressive sensing (CS) when the sizes of the unknown part of the support and of errors in the known part are small compared to the support size. An important extension called Regularized Modified-CS (RegModCS) is developed which also uses prior signal estimate knowledge. Simulation comparisons for both sparse and compressible signals are shown.

==> fig1.tex <==

\begin{figure*}[h]
\vspace{-0.3in}
\centerline{
%\subfigure[Static Problem]{\label{modcssim}
\begin{tabular}{cc}
\includegraphics [height=6cm, width=9cm]{LLsparseheartFT19obsnoiselessrecon3separate.eps} &
\includegraphics [height=6cm, width=9cm]{LLsparseheartGauss29obsnoiselessrecon3separate.eps}
\vspace{-1in}\\
\small{(a) Fourier meas.} & \small{(b) Gaussian meas.}
\end{tabular}
%}
}
\caption{\small{(a) Reconstructing a $32 \times 32$ sparsified cardiac image ($m=1024$) from $n = 0.19m=195$  random Fourier measurements. Support size $|T \cup \Delta| = 107$ and  $|T|=64$.
. Modified-CS achieved exact reconstruction, while the normalized CS reconstruction error was 13\%.
 %We used the lowest subband of a 2-level wavelet decomposition as the known part of the support, $T$. Thus,
%The image used here is a sparsified one: take wavelet transform of original image, retain the largest 107 coefficients (corresponds to $99\%$ of image energy) and take inverse wavelet transform.
(b) Reconstruction using $n = 0.29m$ random Gaussian measurements. Modified-CS achieved exact reconstruction, while the normalized CS reconstruction error was 34\%.
}}
\vspace{-0.15in}
\label{static}
\end{figure*}





==> fig2.tex <==
\begin{figure*}
\centerline{
%\subfigure[Top: Sparse, Bottom: Real]{\label{timeseq_plots}
\begin{tabular}{cc}
\includegraphics [height=6cm,width=8cm]{sparseheartFTWT16obsnoiseless2.eps} &
\includegraphics [height=6cm,width=8cm]{heartGauss19obsnoiseless2_mod.eps} \\
\small{(a) Sparsified seq, Fourier meas} & \small{(b) Real seq, Gaussian meas}
\end{tabular}
%}
%\hspace{-0.2in}
%\subfigure[Recon. images (sparse)]{\label{timeseq_recon}
%\begin{tabular}{c}
%\includegraphics [height=1.2cm,width=4cm]{C:/Code/KFCS/weilu_fig/noiselessFTsparsifyheart16obs_original.eps} \\
%\includegraphics [height=1.2cm,width=4cm]{C:/Code/KFCS/weilu_fig/noiselessFTsparsifyheart16obs_SeqCS.eps} \\
%\includegraphics [height=1.2cm,width=4cm]{C:/Code/KFCS/weilu_fig/noiselessFTsparsifyheart16obs_CS.eps}
%\end{tabular}
%}
}
%\vspace{-0.1in}
\caption{\small{(a) Exact reconstruction of a sparsified cardiac sequence from only  $n=0.16 m$ random Fourier measurements (MR imaging). Support size, $|N_t|\approx 0.1 m$,size of support change $|\Delta|\approx 1\%$ of $m$. %Image size was $32 \times 32$, i.e. $m=1024$.
Simple CS (referred to as CS in the figure) has very large (20-25\%) error while modified-CS gives exact reconstruction. (b) Reconstructing a real cardiac sequence from $n=0.19 m$ random Gaussian measurements.
}}% for $t>1$
% from noiseless Fourier measurements (MR imaging) . Support,  $|N_t|\approx 10\%$.  for $t>1$
%\vspace{-0.45in}
\label{timeseq}
\end{figure*}


%\begin{figure}
%\centerline{
%%\subfigure[Static Problem]{\label{modcssim}
%%\begin{tabular}{c}
%%\includegraphics [height=4cm]{C:/Code/KFCS/weilu_fig_jan09/LLsparseheartFT19obsnoiselessrecon3separate.eps} \\
%%\includegraphics [height=4cm]{C:/Code/KFCS/weilu_fig_jan09/LLsparseheartGauss29obsnoiselessrecon3separate.eps}
%%\end{tabular}
%%}
%\subfigure[Top: Sparse, Bottom: Real]{\label{timeseq_plots}
%\begin{tabular}{c}
%\includegraphics [height=2cm,width=4.5cm]{C:/Code/KFCS/weilu_fig/sparseheartFTWT15obsnoiseless2.eps} \\
%\includegraphics [height=2cm,width=4.5cm]{C:/Code/KFCS/weilu_fig/heartGauss19obsnoiseless2_mod.eps}
%\end{tabular}
%}
%\hspace{-0.2in}
%\subfigure[Recon. images (sparse)]{\label{timeseq_recon}
%\begin{tabular}{c}
%\includegraphics [height=1.2cm,width=4cm]{C:/Code/KFCS/weilu_fig/noiselessFTsparsifyheart16obs_original.eps} \\
%\includegraphics [height=1.2cm,width=4cm]{C:/Code/KFCS/weilu_fig/noiselessFTsparsifyheart16obs_SeqCS.eps} \\
%\includegraphics [height=1.2cm,width=4cm]{C:/Code/KFCS/weilu_fig/noiselessFTsparsifyheart16obs_CS.eps}
%\end{tabular}
%}
%}
%\vspace{-0.1in}
%\caption{\small{(a) Top: Exact reconstruction of a sparsified cardiac sequence from only  $n=0.16 m$ random Fourier measurements (MR imaging). Support size, $|N_t|\approx 0.1 m$. Image size was $32 \times 32$, i.e. $m=1024$. Simple CS (referred to as CS in the figure) has very large (20-25\%) error while modified-CS gives exact reconstruction. Bottom: Reconstructing a real cardiac sequence from $n=0.19 m$ random Gaussian measurements.
%(b) Some sample reconstructed images.
%}}% for $t>1$
%% from noiseless Fourier measurements (MR imaging) . Support,  $|N_t|\approx 10\%$.  for $t>1$
%\label{timeseq}
%\end{figure}


%\begin{figure*}
%\centerline{
%\subfigure[mod-CS-recursive]{\label{modcsdiag}
%\epsfig{file = U:/Proposals/Dec08/modifiedCS2.eps, width = 7cm} %,height=4cm,width=6cm}
%}
%\subfigure[modified-CS versus regular CS (CS)]{\label{modcssim}
%%\includegraphics [height=41mm,width=47mm]{sparseheartBER16obsnoiseless.eps}
%\includegraphics [height=3.5cm,width=6cm]{C:/Code/KFCS/weilu_fig/sparseheartFTWT15obsnoiseless2.eps}
%%\includegraphics [height=2cm,width=7cm]{C:/Code/KFCS/weilu_fig/noiselessFTsparsifyheart16obs_original.eps} \\
%%\includegraphics [height=2cm,width=7cm]{C:/Code/KFCS/weilu_fig/noiselessFTsparsifyheart16obs_SeqCS.eps} \\
%%\includegraphics [height=2cm,width=7cm]{C:/Code/KFCS/weilu_fig/noiselessFTsparsifyheart16obs_CS.eps}
%}
%}
%\vspace{-0.1in}
%\caption{\small{ (a) Recursive Reconstruction using modified-CS. (b) Exact reconstruction of a sparsified cardiac sequence from only  $n=16\%$ Fourier measurements (MR imaging). Support size, $|N_t|\approx 10\%$. Image size was $32 \times 32$, i.e. $m=1024$. Regular CS (referred to as CS in the figure) has very large (20-25\%) error while modified-CS gives exact reconstruction.}}% for $t>1$
%% from noiseless Fourier measurements (MR imaging) . Support,  $|N_t|\approx 10\%$.  for $t>1$
%\end{figure*}


==> modcs_algo.tex <==
\section{Modified Compressive Sensing (mod-CS)}
%At time, $t$, we have an estimate of the signal from $t-1$, and hence of its support, $\Nhat_{t-1}$. Let $T := \Nhat_{t-1}$.
Our goal is to find the sparsest possible signal estimate whose support contains $T$ and which satisfies the data constraint (\ref{obsmod}), i.e. %We need to find the unknown part of the support, $\Delta$, so that the resulting signal estimate is the sparsest possible. %and the coefficient estimates along $T$ and $\Delta$.
%In other words, %we would like to find a solution with the minimum number of new additions to the set $T$ and that satisfies the data constraint, i.e.
we would like to find a $\hat{x}$ which solves %, i.e. we would like to minimize the $\ell_0$ norm of the newly added coefficients' vector subject to the data constraint, i.e. compute
\bea
\min_\beta  ||(\beta)_{T^c}||_0 \ \text{subject to} \ y = A \beta
\label{l0seqcs}
\eea
where $T^c : = [1:m] \setminus T$ denotes the complement of $T$.

As is well known, minimizing the $\ell_0$ norm has combinatorial complexity. We propose to use the same trick that resulted in compressive sensing. We replace the $\ell_0$ norm by the $\ell_1$ norm, which is the closest norm to $\ell_0$ that makes the optimization problem convex, i.e. we solve %Thus at each time $t$, we solve
\bea
\min_\beta  ||(\beta)_{T^c}||_1 \ \text{subject to} \ y = A \beta
\label{l1seqcs}
\eea

%As we show later, this achieves exact reconstruction using much fewer observations than those required for regular CS.

%The support at $t$, $\Nhat_t$ is computed by thresholding  $\xhat_{t,\text{modCS}}$. A block diagram is given in Fig. \ref{modcsdiag}.


\subsection{Recursive Reconstruction of Signal Sequences}
Consider the recursive reconstruction problem where $y \equiv y_t$ and $x \equiv x_t$ with support $N \equiv N_t$. The known part of the support, $T =  \hat{N}_{t-1}$. In this case, at each time, $t$, we solve (\ref{l1seqcs}) and denote its output by $\xhat_{t,\text{modCS}}$. The support at $t$, $\Nhat_t$ is computed by thresholding  $\xhat_{t,\text{modCS}}$, i.e.
\bea
\Nhat_t = \{i \in [1:m] : (\xhat_{t,\text{modCS}})_i^2 > \alpha \}
\eea
where $\alpha$ is a small threshold (ideally zero). With this we automatically estimate $\hat{\Delta} = \Nhat_t \setminus T$ and $\hat{\Delta}_d = T \setminus \Nhat_t$.

A block diagram of our proposed approach is given in Fig. \ref{modcsdiag}.
Our experiments suggest that doing the above gives exact reconstruction using much fewer measurements than those required for CS at each time (simple CS), see Fig. \ref{timeseq}. Here the support of $x_t$ was about $10\%$ of the image size, while we were able to get {\em exact reconstruction} using as few as $n=16\%$ observations. The reason was that the size of the change in the support from $t-1$ to $t$, $|\Delta|$, was $1\%$ or less. Clearly, with so few observations, simple CS does not work. %Note that at $t=1$, both algorithms perform CS and used enough observations for CS to give exact reconstruction.

%\begin{figure}[t!]
%\centerline{
%\epsfig{file = U:/Proposals/Dec08/modifiedCS2.eps, width = 7cm}% height = 2cm} %,height=4cm,width=6cm}
%}
%\vspace{-0.15in}
%\caption{\small{Modified-CS for time sequence reconstruction
%}}
%\vspace{-0.15in}
%\label{modcsdiag}
%\end{figure}

